Spectral Filtering for General Linear Dynamical Systems

We give a polynomial-time algorithm for learning latent-state linear dynamical systems without system identification, and without assumptions on the spectral radius of the system's transition matrix. The algorithm extends the recently introduced technique of spectral filtering, previously applied only to systems with a symmetric transition matrix, using a novel convex relaxation to allow for the efficient identification of phases.

==> ICML18/A01-appx.tex <==
\section{Proof of approximation theorem}
\label{app:approx}

Note that throughout the paper, we can assume without loss of generality that $D = 0$ (the zero matrix) for any LDS we wish to approximate. When this is not the case, we simply add an autoregressive component with delay zero $P_0$, which increases the norm of the pseudo-LDS by an additive $R_\Theta$.

\subsection{Warm-up: Simple autoregressive model}
\label{sec:ar}

As a warm-up, we first establish rigorous regret bounds for an autoregressive model, depending on properties of the the minimal polynomial of the linear dynamical system. Next we will see how introducing wavefilters can improve these bounds.

\begin{theorem}\label{thm:arma}
Consider a LDS $\Te=(A,B,C, h_0=0)$, where $A=\Psi \La \Psi^{-1}$ is diagonalizable with spectral radius $\le 1$.
Let $p(x)$ be a monic polynomial of degree $\tau$ such that $p(A)=0$.\footnote{In other words, the minimal polynomial of $A$ divides $p$. For a diagonalizable matrix, the minimal polynomial is the characteristic polynomial except without repeated zeros.}
 Suppose %$\ve{p}_2\le R$, 
 $\ve{p}_1\le R_1$,\footnote{For a polynomial $p(x) = \sumz j{\tau} \be_{j}x^{\tau-j}$, let
\begin{align}
\ve{p}_1 &= \sumz j{\tau} |\be_{j}|
\end{align}} $\ve{B}_2,\ve{C}_2\le R_\Te$, and $\ve{\Psi}_F\ve{\Psi^{-1}}_F\le R_\Psi$. 

Suppose $y_1,\ldots, y_t$ is generated from the LDS with inputs $x_t$. Then there exist $\be\in \R^\tau$ and $P_0,\ldots, P_{\tau-1}\in \R^{m\times n}$ satisfying
\begin{align}\label{eq:arma-cons1}
\ve{\be}_1 &\le R_1%-1
\\
\label{eq:arma-cons2}
\ve{P_j}_F &\le R_1 R_\Te^2 R_\Psi
\end{align}
such that
\begin{align}
y_t & = -\sum_{j=1}^{\tau} \be_j  y_{t-j} + \sum_{j=0}^{\tau-1} P_j x_{t-j}.
\end{align}
\end{theorem}
\begin{proof}
Unfolding the LDS,
\begin{align}
y_t &=\sumz i{t-1} CA^iB x_{t-i} % + CA^t h_0
\\
%y_{t-d+j} &= \sumz i{t-d+j-1}CA^i B x_{t-d+j-i}\\
%&=\sum_{i=d-j}^{t-1} CA^{j-d+1}x_{t-i}
y_{t-j} &= \sumz i{t-j-1} CA^iB x_{t-j-i} % + CA^{t-j} h_0
=\sum_{i=j}^{t-1} CA^{i-j}B x_{t-i}.
\end{align}
Let $p(x) = \sumz j{\tau} \be_{j}x^{\tau-j}$ (with $\be_0=1$).  Then
\begin{align}
&\sumz j{\tau} \be_j  y_{t-j} \\
=& \sumr{0\le j\le \tau}{j\le i\le t-1} \be_j  CA^{i-j} Bx_{t-i} \\
=&\sumz i{\tau-1} \sum_{j=0}^i \be_j  CA^{i-j} Bx_{t-i} + \ub{C\sum_{i=\tau}^{t-1} \pa{\sumz j{\tau} \be_j  A^{i-j}}Bx_{t-i}}{=0}\label{eq:char-poly-y}
\end{align}
using the fact that 
$\sum_{j=0}^{\tau} A^{i-j} = A^{i-j-\tau} p(A)=0$. Writing this in the autoregressive format,
\begin{align}
y_t &= -\sumo j{\tau} \be_j  y_{t-j} + C\sumz i{\tau-1} \sum_{j=0}^i \be_j  CA^{i-j} Bx_{t-i}.
\end{align}
We let $N_i = \sum_{j=0}^i \be_j  CA^{i-j}B$ for $0\le i\le \tau-1$ and check that this satisfies the conditions. Note $\ve{MN}_F\le \min\{\ve{M}_2\ve{N}_F,\ve{M}_F\ve{N}_2\}$. By the $L^1$-$L^\iy$ inequality,
\begin{align}
&\ve{P_i}_F \\
=&\ve{\sumz ji \be_j  CA^{i-j} B}_F\\
%&\le \pa{\sumz ji \be_j ^2}\pa{\sumz ji \ve{CA^{i-j} B}_F^2}\\
\le& \pa{\sumz ji |\be_j |} \max_{0\le j\le i} \ve{CA^{i-j}B}_F\\
\le& R_1 \ve{C}_2\ve{\Psi}_F \ve{\La}_2\ve{\Psi^{-1}}_F\ve{B}_2\\
\le& R_1 R_\Te^2 R_\Psi.
%\le R^2R_\Te^2.
\end{align}
\end{proof}

\subsection{Autoregressive model with wavefilters: An approximate convex relaxation for asymmetric LDS}
\label{app:ar-wave}

If we add wavefiltered inputs to the regression, the bounds depend not on the minimal polynomial $p$ of $A$, but rather on the minimal polynomial having all the $\om_\ell$ as zeros, where $\om_\ell$ are the phases of zeros of the characteristic polynomial of $A$. For example, if all the roots are real and distinct, then the polynomial is $x-1$ rather than $\prod_{p(\al)=0} (x-\al)$. This can be an exponential improvement. For example, consider the case where all the $\al$ are close to 1. Then the minimal polynomial is close to $(x-1)^d$, which has coefficients as large as $\exp(\Om(d))$. Note the case of real roots reduces to~\cite{HKZ17}.

First, we introduce some notation for convenience. Note that in~\eqref{eq:pseudo-LDS}, $\sumo uT \phi_h(u) x_{t-u}(i) \cos\pf{2\pi u p}{W}$ is a certain convolution. For $a\in \R^T$ we define
\begin{align}
a^{(\om)}:&= (a_j \om^j)_{1\le j\le T}\\
a^{(\cos,\te)} :&= (a_j \cos(j\te))_{1\le j\le T}\\
a^{(\sin,\te)} :&= (a_j \sin(j\te))_{1\le j\le T}.
\end{align}
so that we can write~\eqref{eq:pseudo-LDS} as
\begin{align}\label{eq:pseudo-LDS2}
 &y(M, N,\beta,P; x_{1:t}, y_{t-1:t-d}) \\
 =& \sum_{u=1}^\tau \beta_u y_{t-u} +
\sumz j{\tau-1} P_j x_{t-j} \\
& + 
\sum_{p=0}^{P-1} 
\sum_{h=1}^k 
\sum_{u=1}^T 
\Bigg(M(p,h,:,:)
\si_h^{\rc 4}(\phi_h^{(\cos, \fc{2\pi u p}{P})} * x)_{t-\tau} \\
& \quad+
N(p,h,:,:)
\si_h^{\rc 4}
(\phi_j^{(\sin, \fc{2\pi u p}{P})} * x)_{t-\tau}\Bigg)  
 \end{align}
 
 We now give a more precise statement of Theorem~\ref{thm:arma-wf} and prove it.
 \begin{theorem}\label{thm:arma-wf-precise}
Consider a LDS $\Te=(A,B,C, h_0=0)$, where $A$ is diagonalizable with spectral radius $\le 1$.
Let the eigenvalues of $A$ be $\al_\ell = \omega_\ell r_\ell$ for $1\le \ell\le d$, where $|\omega_\ell|=1$ and $r_\ell\in \R_{\ge 0}$. Let $S$ be the set of $\om_\ell$. %\footnote{\fixme{Can relax this further---each $\om_\ell$ is within some small enough $\ep$ of an element of $S$.}} 
Let $p(x)$ be a monic polynomial of degree $\tau$ such that $p(\om_\ell)=0$ for each $\ell$.
Suppose $\ve{p}_1\le R_1$, 
 $\ve{B}_2,\ve{C}_2\le R_\Te$,
 and the diagonalization $A=\Psi \La \Psi^{-1}$ satisfies $\ve{\Psi}_F\ve{\Psi^{-1}}_F\le R_\Psi$.

Suppose $y_1,\ldots, y_T$ is generated from the LDS with inputs $x_1,\ldots, x_T$ such that $\ve{x_t}_2\le R_x$ for all $1\le t\le T$.
Then 
there is $k=O\pa{
\ln T \ln \pf{\tau R_\Te R_\Psi R_1 R_xT}{\ep}
}$, $P=O\pf{\tau R_\Te^2 R_\Psi R_1R_xT^{\fc 32}}{\ep}$, 
$M,N\in \R^{W\times k\times n\times m}$, $\be\in \R^\tau$ and $P_0,\ldots, P_{\tau-1}\in \R^{m\times n}$ satisfying
\begin{align}\label{eq:arma-wf-cons1}
\ve{\be}_1 &\le R_1
\\
\label{eq:arma-wf-cons2}
\ve{P_j}_F &\le R_1 R_\Te^2 R_\Psi\\
\label{eq:arma-wf-cons3}
\sqrt{\ve{M}_{2,1}^2 + \ve{N}_{2,1}^2}&=O(R_\Te^2R_\Psi R_1\tau k^{\rc 2})
\end{align}
such that 
the pseudo-LDS $(M,N,\be, P)$ approximates $y_t$ within $\ep$ for $1\le t\le T$:
\begin{align}
\ve{y(M,N,\be,P_{0:\tau-1}; x_{1:t}, y_{t-1:t-\tau})-y_t}&\le \ep.
\end{align}
\end{theorem}


\begin{proof} %[Proof of Theorem~\ref{thm:arma-wf}]
Our plan is as follows. First we show that choosing $\be_j$ and $P_j$ as in Theorem~\ref{thm:arma}, 
\begin{align}
\de_t &= y_t + \sum_{j=1}^{\tau} \be_j  y_{t-j} - \sum_{j=0}^{\tau-1} P_j x_{t-j} 
\end{align}
 can be approximated by 
\begin{align}
\de_t^{(1)} :&= \sum_{\ell=1}^d 
 \sum_{h=1}^k
M_\ell'(h,:,:) \si_h^{\rc 4}(\phi_h^{(\om_\ell)}*x)_{t-\tau}
\end{align}
for $M_\om'\in \R^{k\times n\times m}$; this is obtained by a projection to the wavefilters. Next we approximate $\de_{t}^{(1)}$ by discretization of the phase,
\begin{align}
\de_t^{(2)} :&= \sum_{\ell=1}^{d}
 \sum_{h=1}^k
M_\ell'(h,:,:) \si_h^{\rc 4}(\phi_h^{(e^{2\pi i p_\ell/W})}*x)_{t-\tau}
\end{align}
for some integers $p_\ell\in [0,W-1]$. 
Finally, we show taking the real part gives something in the form
\begin{align}
\sum_{\ell=1}^{d}
\sum_{h=1}^k %\sum_{h=1}^k
%\sum_{u=1}^{t-\tau}
 \Bigg(M_\ell(h,:,:)\si_h^{\rc 4} (\phi_h^{(\cos, \fc{2\pi p_\ell}{W})}*
x)_{t-\tau}\\
+(N_\ell(h,:,:)\si_h^{\rc 4} (\phi_h^{(\sin, \fc{2\pi p_\ell}{W})}*
x)_{t-\tau}\Bigg)
\label{eq:real-part}
\end{align}
This matches the form of a pseudo-LDS given in~\eqref{eq:pseudo-LDS} after collecting terms, 
\begin{align}
M(p,:,:,:) &= \sum_{\ell:p_\ell=p} M_\ell&
N(p,:,:,:) &= \sum_{\ell:p_\ell=p} N_\ell.
\end{align}

Now we carry out the plan. Again we have~\eqref{eq:char-poly-y} except that this time the second term is not 0. Let $A=\Psi\La \Psi^{-1}$, $v_\ell$ be the columns of $\Psi$ and $w_{\ell}^*$ be the rows of $\Psi^{-1}$.
By assumption on $p$, $\sumz j{\tau} \be_j \om_\ell^{\tau-j}=0$ for each $\ell$, so the second term of~\eqref{eq:char-poly-y} equals
\begin{align}
&\de_t \\
=& C\sum_{i=\tau}^{t-1} \pa{\sum_{\ell=1}^d \sumz j{\tau} \be_j  \al_\ell^{i-\tau}\al_\ell^{\tau-j} v_\ell w_\ell^*}Bx_{t-i} \\
=&
C\sum_{i=\tau}^{t-1} \pa{\sum_{\ell=1}^d \al_\ell^{i-\tau}\sumz j{\tau} \be_j  (\al_\ell^{\tau-j} - \om_\ell^{\tau-j}) v_\ell w_\ell^*}Bx_{t-i}\\
=&\sum_{\ell=1}^dCv_\ell w_\ell^*B \sum_{i=\tau}^{t-1} r_\ell^{i-\tau}\om_\ell^{i-\tau} \sumz j{\tau}  \be_j \om_\ell^{\tau-j} (r_\ell^{\tau-j}-1) x_{t-i}\\
=& \sum_{\ell=1}^dCv_\ell w_\ell^*B \sumz j{\tau}  \sum_{i=\tau}^{t-1} \be_j  \pa{r_\ell^{\tau-j}-1} r_\ell^{i-\tau}
\om_\ell^{i-j}x_{t-i}\\
=&\sum_{\ell=1}^dCv_\ell w_\ell^*B  \sumz j{\tau}  \be_j  \om^{\tau-j} \fc{r^{\tau-j}-1}{1-r} \pa{\mu(r_\ell)^{(\om_\ell)}*x}_{t-\tau}.
\end{align}

Thus this equals
\begin{align}
%&=\sum_{\ell=1}^dCv_\ell\ot w_\ell^*B \sumz j{\tau}  \be_j  \pa{\fc{1-r^{\tau-j}}{1-r}\mu_1(r_\ell)*x^{(\om_\ell)}}_{t-\tau}\\
&\de_t \\
=&
\ub{\sum_{\ell=1}^dCv_\ell w_\ell^*B \sumz j{\tau}  \be_j  \om_\ell^{\tau-j} \fc{r^{\tau-j}-1}{1-r} \pa{\wt \mu(r_\ell)^{(\om_\ell)}*x}_{t-\tau}}{\de_t^{(1)}}
\label{eq:arma-wave-term1}
\\
&+
\sum_{\ell=1}^dCv_\ell w_\ell^*B \sumz j{\tau}    \be_j  \om_\ell^{\tau-j} \fc{r^{\tau-j}-1}{1-r} \\
& \quad \quad \quad \quad \quad \quad \quad \quad \pa{(\mu(r_\ell)-\wt \mu(r_\ell))^{(\om_\ell)}*x}_{t-\tau}%{\ep_t^{(1)}}\label{eq:arma-wave-error}
\end{align}
where $\wt \mu_k(r)$ is the projection of $\mu_k(r)$ to the subspace spanned by the rows of $\phi_1,\ldots, \phi_k$. %, i.e., 
Let $\Phi$ be the matrix with rows $\phi_j$, let $D=\diag((\si_h^{\rc 4})_{1\le h\le k})$ and let $m_\ell\in \R^k$ be such that $\wt \mu(r_\ell) = \Phi Dm_\ell = \sum_{h=1}^k m_{\ell,h}\si_h^{\rc 4}\phi_h$, i.e., $m_\ell = \si_h^{-\rc 4} \an{\phi_h,\mu(r_\ell)}$. The purpose of $D$ is to scale down $\phi_h*x$ so that gradients will be small in the optimization analysis.

We show that the term~\eqref{eq:arma-wave-term1} equals $\de_t^{(1)}$ with some choice of $M_\ell'$. 

\begin{align}
&\eqref{eq:arma-wave-term1}\\
=& \sumo{\ell}d Cv_\ell w_\ell^* B \sumz j{\tau-1} \be_j  \om_\ell^{\tau-j} \fc{r^{\tau-j}-1}{1-r}\\
& \quad \quad \quad \quad \quad \quad \quad \quad \sum_{h=1}^k m_{\ell,h}\si_h^{\rc 4}(\phi_{h}^{(\om_\ell)}* x)_{t-\tau}\\
=&\sumo{\ell}{d}
 \sum_{h=1}^k
 M_\ell'(h,:,:) \si_h^{\rc 4}(\phi_h^{(\om_\ell)} * x)_{t-\tau}\\
=&\de_t^{(1)}
\end{align}
where $M_\ell' (h,r,i):=(L_\ell)_{ri} m_{\ell,h}$ and 
\begin{align}
L_\ell&= Cv_\ell w_\ell^*B \sumz j{\tau-1} \be_j  \om_\ell^{\tau-j} \pf{r^{\tau-j}-1}{1-r} 
\end{align}
We calculate the error. Here $\ve{x}_\iy$ denotes $\max_i \ve{x_i}_2$.
\begin{align}
&\sumo{\ell}d \ve{L_\ell}_F \\
=&\sumo{\ell}d
\ve{Cv_\ell w_\ell^* B\sumz j{\tau-1} \be_j \om_\ell^{\tau-j}
\fc{r^{\tau-j}-1}{1-r}
}_F\\
\le& \sumo{\ell}d \ve{C}_F\ve{B}_F \ve{v_\ell}_2\ve{w_\ell}_2\ve{\be}_1\tau\\
\le& \ve{C}_F\ve{B}_F \sqrt{\sumo{\ell}d\ve{v_\ell}_2^2\sumo{\ell}d\ve{w_\ell}_2^2}\ve{\be}_1\tau
\label{eq:RPsi}\\
\le& R_\Te^2R_\Psi R_1\tau
\label{eq:L-bound}
\\
&\ve{\de_t-\de_t^{(1)}}_2 \\
 \le &
\sumo{\ell}d \ve{L_\ell}_2
\max_\ell ((\mu(r_\ell) - \wt \mu(r_\ell))^{(\om_\ell)} * x)_{t-\tau}\\
\le& R_\Te^2R_\Psi R_1\tau
\max_\ell \ve{\mu(r_\ell)-\wt \mu(r_\ell)}_1\ve{x}_{\iy}\\ %can actually improve to \sqrt{\tau}
\le& R_\Te^2R_\Psi R_1\tau \sqrt{T}\max_\ell\ve{\mu(r_\ell)-\wt \mu(r_\ell)}_2R_x\\
\le& R_\Te^2R_\Psi R_1\tau \sqrt T c_1^{-k/\ln T}(\ln T)^{\rc 4}.
\end{align}
for some constant $c_1<1$, where the bound on $\ve{\mu(r_\ell)-\wt \mu(r_\ell)}$ comes from Lemma C.2 in \cite{HKZ17}. Choose $k=C\ln T \ln \pf{\tau R_\Te R_\Psi R_1R_x T}{\ep}$ for large enough $C$ makes this $\le \eph$. 

Now we analyze the effect of discretization. Write $\om_\ell = e^{\te_\ell i}$ where $\te_\ell \in [0,2\pi)$, and let $p_\ell$ be such that 
$\ab{\te_\ell - \fc{2\pi p_\ell}{W}}\le \fc{\pi}{W}$ where the angles are compared modulo $2\pi$. 
Let $\om_\ell'=e^{\fc{2\pi p_\ell i}{W}}$. 
We approximate $\de_t^{(1)}$ with 
\begin{align}
\de_t^{(2)} &= \sumo{\ell}d M_\ell'(h,:,:)\si_h^{\rc 4} (\phi_h^{(\om_\ell')} * x)_{t-\tau}
\end{align}
Note that $|\om_\ell^j - \om_\ell'^j|\le j\ab{\te_\ell - \fc{2\pi p_\ell}W}\le \fc{\pi j}{W}$.
We calculate the error. First note
\begin{align}
\sum_{\ell=1}^d \sumo hk \ve{M_\ell'(h,:,:)}_F\si_h^{\rc 4}
&\le \sumo{\ell}d \ve{L_\ell}_2 \max_{\ell,h} |\an{\phi_h,\mu(r_\ell)}| \\
&\le R_\Te^2R_\Psi R_1\tau
\end{align}
by \eqref{eq:L-bound} and $\ve{\mu(r_\ell)}_2\le 1$. Then
\begin{align}
&\ve{\de_t^{(1)} - \de_t^{(2)}}_2 \\
\le& \sumo hk \ve{\sumo{\ell}d M_\ell'(h,i,:) ((\phi_h^{(\om_\ell)} - \phi_h^{(\om_\ell')})*x)_{t-\tau}(i)}_2\\
\le& \pa{\sum_{\ell=1}^d \sumo hk \ve{M_\ell'(h,:,:)}_F\si_h^{\rc 4}}
\max_{h,\ell} \ve{\phi_h^{(\om_\ell)}-\phi_h^{(\om_\ell')}}_1 R_x\\
\le& R_\Te^2R_\Psi R_1\tau \fc{\pi T}{W}\max_h \ve{\phi_h}_1 R_x\\
\le& R_\Te^2R_\Psi R_1\tau \fc{\pi T}{W} \sqrt{T} R_x\\
=& \fc{R_\Te^2R_\Psi R_1\tau\pi T^{\fc 32} R_x}{W}\le\eph
\end{align}
for $W=\fc{2\pi \tau R_\Te^2 R_\Psi R_1R_x T^{\fc 32}}{\ep}$. This means $\ve{\de_t-\de_t^{(2)}}\le \ep$.

Finally, we take the real part of $ \de_t^{(2)}$ (which doesn't increase the error, because $\de_t$ is real)
to get 
\begin{align}
%\sumo uT \phi_j(u) x_{t-u}(i) M_\ell(r,i,j) \om_\ell^u
& \quad 
\sumo{\ell}d
\sum_{i=1}^n \sum_{h=1}^k
\sumo uT \si_h^{\rc 4}\phi_h(u) x_{t-\tau-u}(i) \Re [M_{\ell}'(h,:,i){\om_\ell'}^u]\\
&= \sumo{\ell}d 
\sum_{i=1}^n \sum_{h=1}^k
\sumo uT \si_h^{\rc 4}\phi_h(u) x_{t-\tau - u}(i)\Bigg(\Re(M_{\ell}'(h,:,i)) \\
& \quad \cos\pf{2\pi p_\ell u}{W} - 
\Im(M_{\ell}'(h,:,i)) \sin\pf{2\pi p_\ell u}{W} 
\Bigg)
%&=\sumo{\ell}d\sumo uT \phi_j(u) x_{t-u}(i)
%|M_{\om_\ell'}(r,i,j)| (\cos(\te_{\ell,r,i,j}) \cos(u\te_\ell) - \sin(\te_{\ell,r,i,j}) \sin(u\te_\ell))\\
\end{align}
which is in the form~\eqref{eq:real-part} with $M_\ell = \Re(M_\ell')$ and $N_\ell =-\Im(M_\ell')$.

The bound on $\ve{M}_{2,1}$ and $\ve{N}_{2,1}$ is
\begin{align}
&\quad \sqrt{\ve{M}_{2,1}^2 + \ve{N}_{2,1}^2}\\
&\le \sumo{\ell}d \sqrt{\ve{M_\ell}_F^2 + \ve{N_\ell}_F^2}= \sumo{\ell}d \ve{M_\ell'}_F \\
&=\sumo{\ell}d \sqrt{\sumo hk \ve{M_\ell'(h,:,:)}_F^2}\\
&=\sumo{\ell}d \ve{L_\ell}_F \ve{m_\ell}_2\\
&= O(R_\Te^2R_\Psi^2R_1\tau k^{\rc 2})
\end{align}
because \begin{align}
\ve{m_\ell}_2 &=\pa{\sumo hk \si_h^{-\rc 2} \an{\phi_h, \mu(r_\ell)}^2}^{\rc 2}\\
&\le\pa{\sumo hk O(1)}^{\rc 2}=O(k^{\rc 2})
\end{align}
by Lemma E.4 in~\cite{HKZ17}.
\end{proof}

%\subsection{Approximating the moment curve}
%This approximation result is a variant to Lemma 4.1 from \cite{HKZ17}, and follows
%the same proof structure; we include it for sake of completeness.
%It governs the low-rank approximation for the \emph{moment curve} $\mu(\alpha) \in \reals^T$,
%defined by the vector of successive powers $[1 \; \alpha \; \ldots \; \alpha^{T-1}]^\top$.
%Note that \cite{HKZ17} obtains an approximation guarantee on $(1-\alpha) \mu(\alpha)$.
%The Hilbert matrix $H_T$ arises as the second moment matrix of the distribution $\mu(\alpha)$ for a uniform choice of $\alpha$.
%\begin{lemma}[Low-rank approximation of the moment curve]
%\label{lem:moment-curve-appx}
%Let $\alpha \in [0,1]$. Let $\Pi_k \in \R^{T \times k}$ be the matrix whose columns are the top $k$ eigenvectors of the Hilbert matrix $H_T$. Then, we have
%\[ \norm{ (I - \Pi_k\Pi_k^\top) \mu(\alpha) }_2 \leq O\left( c_0 ^ {-k/\log T} \sqrt{T} \log^{1/4} T \right), \]
%for an absolute constant $c_0$, for all $T \geq 10$.
%\end{lemma}
%\begin{proof}
%Let $r(\alpha) := (I - \Pi_k\Pi_k^\top) \mu(\alpha)$ denote the residual.
%We have
%\begin{align*}
%\E_{\alpha \sim \mathrm{Unif}([0,1])} [ \norm{ r(\alpha) }^2 ] = \trace \int_0^1 (I - \Pi_k\Pi_k^\top) \mu(\alpha) \mu(\alpha)^\top \, d\alpha = \sum_{j=k+1}^T \sigma_j.
%\end{align*}
%Corollary 4.2 of \cite{beckermann2017singular} gives a bound on the rate of spectral decay of the Hilbert matrix. In particular, we have, for $T \geq 10$,
%\[ \sigma_{k+1}(H_T) \leq c_1 \cdot c_2 ^ {-k/\log T} \]
%for some absolute constants $c_1, c_2$.
%This implies
%\[ \E [ \norm{ r(\alpha) }^2 ] \leq O\left(c_1 ^ {-k / \log T} \cdot \log T \right). \]
%Now, as in the proof of Lemma C.2, to translate the expected reconstruction error bound into one that is uniform for all $\alpha$, we bound the Lipschitz constant of $r(\alpha)$:
%\begin{align*}
%|\frac{d}{d\alpha} \norm{ r(\alpha) }^2| \leq |\frac{d}{d\alpha} \norm{ \mu(\alpha) }^2|
%= \frac{d}{d\alpha} \sum_{t=0}^{T-1} \alpha^{2t}
%= \sum_{t=0}^{T-1} 2t \alpha^{2t-1} < T^2.
%\end{align*}
%Thus we conclude
%\begin{align*}
%\max_{\alpha \in [0,1]} \norm{ r(\alpha) }^2 \leq \sqrt{ 2 T^2 \sum_{j=k+1}^T \sigma_j }
%\leq O\left(c_0^{-k / 2\log T} T \sqrt{\log T} \right),
%\end{align*}
%which implies the claim.
%\end{proof}
%
%\subsection{Approximate convex relaxation for asymmetric LDSs}
%\begin{theorem}
%Let $\Theta = (A,B,C,D)$ be the parameters for an LDS, with $\norm{A}_2 \leq 1$ and $\norm{B}_F, \norm{C}_F, \norm{D}_F \leq R_\Theta$. Then, with a choice of filter parameter $k = \Theta(\log T \log (R_x R_\Theta R_\Psi n T/\eps ))$ and phase discretization parameter $P = \Omega(d T^2 R_x R_\Theta^2 R_\Psi^2 / \eps)$, there exists some $M_\Theta$ for whose predictions are all close to those of $\Theta$ on all inputs:
%\[\norm{ y(M_\Theta; x_{1:t}) - y_t } \leq \eps, \quad \forall \norm{x_t} \leq R_x. \]
%\end{theorem}
%\begin{proof}
%Let $\Theta = (A,B,C,D=0)$ specify an LDS. We set $D$ to be the zero matrix for clarity of presentation; this only adds a (convex) least-squares linear regression loss, while increasing the norm of $M_\Theta$ by at most a constant factor.
%Write the impulse response function
%\begin{align*}
%y_t &= \sum_{u=1}^T CA^iBx_{t-u}
%= \sum_{u=1}^T C\Phi\bar{A}^u\Phi^{-1}Bx_{t-u} \\
%&= \sum_{u=1}^T \sum_{\ell=1}^d a^u \left[ (C\Phi)_{:,\ell} \otimes (\Phi^{-1}B)_{\ell,:} \right] x_{t-u} \\
%&= \sum_{u=1}^T \sum_{\ell=1}^d |a_\ell|^u e^{i \theta(a_\ell)} \left[ (C\Phi)_{:,\ell} \otimes (\Phi^{-1}B)_{\ell,:} \right] x_{t-u} \\
%&= \sum_{u=1}^T \sum_{\ell=1}^d |a_\ell|^u \left[ \frac{ 1 + 1_{\mathfrak{Im}[a_\ell] \neq 0} }{2} \right] \cos(u \cdot \theta(a_\ell)) \left[ (C\Phi)_{:,\ell} \otimes (\Phi^{-1}B)_{\ell,:} \right] x_{t-u}, \\
%\end{align*}
%where $\theta(\cdot) \in [0, 2\pi)$ denotes the phase of a complex number. The last inequality holds from the fact that $A$ is a real matrix,
%so that the roots of its characteristic polynomial form conjugate pairs.
%For short, denote by $M_{(\ell)}$ the $n$-by-$m$ matrix
%$\left[ (C\Phi)_{:,\ell} \otimes (\Phi^{-1}B)_{\ell,:} \right]$
%We proceed to construct $M_\Theta$ explicitly, in blocks.
%Let $p(a_\ell) = \lfloor \theta(a_\ell)P/2\pi + 1/2 \rfloor$ be the index of the closest phase in the discretization to $\theta(a_\ell)$, and let $I(a_\ell)$ denote the indicator $\frac{ 1 + 1_{\mathfrak{Im}[a_\ell] \neq 0} }{2}$. Then, for all $0 \leq p \leq P-1$, we set:
%\[M(:,:,p,j) =
%\sum_{\ell : p(a_\ell) = p} \langle \mu(|a_\ell|),\phi_j\rangle I(a_\ell) M_{(\ell)}.\]
%We complete the proof by writing the prediction, first applying Lemma~\ref{lem:moment-curve-appx}, which governs the approximation of the time convolutions with the moment curve:
%\begin{align*}
%y(x_{1:t}, M_\Theta) &= \sum_{j=1}^k \sum_{\ell=1}^d \langle \mu(|a_\ell|),\phi_j\rangle I(a_\ell) \cos( 2\pi up(a_\ell)/P ) M_{(\ell)} x_{t-i} \\
%&= \sum_{u=1}^T \sum_{\ell=1}^d |a_\ell|^u I(a_\ell) \cos( 2\pi up(a_\ell)/P ) M_{(\ell)} x_{t-i} \quad + \zeta,
%\end{align*}
%with
%\[\norm{\zeta}_2 \leq 2 \norm{(I-\Pi_k\Pi_k^\top)\mu(a_\ell)}_1 \norm{M_{(\ell)}}_2 R_x \leq O\left(c_2^{-k/\log T} T \log^{1/4} T \sqrt{n} R_\Theta ^2 R_\Psi^2 R_x\right).\]
%Finally, we use the fact that the nearest-phase rounding gives us $| \theta(a_\ell) - 2 \pi p(a_\ell)/P | \leq \pi / P$:
%\begin{align*}
%y(x_{1:t}, M_\Theta) &= \sum_{u=1}^T \sum_{\ell=1}^d |a_\ell|^u I(a_\ell) \cos( 2\pi up(a_\ell)/P ) M_{(\ell)} x_{t-i} \quad + \zeta \\
%&\leq \sum_{u=1}^T \sum_{\ell=1}^d |a_\ell|^u I(a_\ell) \cos( u\theta(a_\ell) ) M_{(\ell)} x_{t-i} \quad + \zeta + \zeta',
%\end{align*}
%with
%\[ \norm{\zeta'}_2 \leq \sum_{u=1}^T \sum_{\ell=1}^d u \norm{M_{(\ell)}}_2 R_x \pi / P \leq O\left( \frac{R_\Theta^2 R_\Psi^2 R_x d T^2}{P} \right). \]
%The stated choices of $k$ and $P$ yield $\norm{\zeta + \zeta'}_2 \leq \eps$, while the double summation term is the impulse response function of $\Theta$.
%\end{proof}


==> ICML18/A02-regret.tex <==
\section{Proof of the regret bound}
\label{section:appendix-regret-proof}

In this section, we prove the following theorem:
\begin{theorem}\label{thm:regret}
Let $y^*_1, \ldots, y^*_T$ denote the predictions made by the fixed pseudo-LDS which has the smallest total squared-norm error in hindsight. Then, there is a choice of parameters for which the decision set $\mathcal{K}$ contains all LDSs which obey the assumptions from Section 2.1,
and Algorithm~\ref{alg:asym-lds} makes predictions $\hat y_t$ such that
\[ \sum_{t=1}^T \norm{\hat y_t - y_t}^2 - \sum_{t=1}^T \norm{\hat y_t^* - y_t}^2 \leq
\tilde O\pa{R d^{5/2} n \log^7 T \sqrt{T}}, \]
where the $\tilde O(\cdot)$ only suppresses factors polylogarithmic in $n,m,d,R_\Theta,R_x,R_y$, and $R_1^3 R_x^2 R_\Theta^4 R_\Psi^2 R_y^2\leq R$.
\end{theorem}

\subsection{Online learning with composite strongly convex regularizers}
\label{subsection:multi-strongly-convex}

Algorithm~\ref{alg:asym-lds} runs the follow-the-regularized-leader (FTRL) algorithm with the regularization
\[ R(M,N,\beta,P) := \norm{M}^2_{2,q} + \norm{N}^2_{2,q} + \norm{\beta}_{q'}^2 + \sum_{j=1}^\tau \norm{P_j}_F^2, \]
where $q = \frac{\ln(W)}{\ln(W)-1}$ and $q' = \frac{\ln(\tau)}{\ln(\tau)-1}$.
To achieve the desired regret bound, we need to show that this regularizer is strongly convex with respect to the composite norm considered in the algorithm. We will work with the following definition of strong convexity with respect to a norm:
\begin{definition}[Strong convexity w.r.t. a norm]
A differentiable convex function $f : \mathcal{K} \rightarrow \reals$ is $\alpha$-strongly convex with respect to the norm $\norm{\cdot}$ if, for all $x, x+h \in \mathcal{K}$, it holds that
\[ f(x+h) \geq f(x) + \langle \nabla f(x),h\rangle + \frac{\alpha}{2} \norm{h}^2. \]
\end{definition}
We first verify the following claim:
\begin{lemma}
\label{lem:multi-strongly-convex-norm}
Suppose the convex functions $R_1, \ldots, R_n$, defined on domains $\mathcal{X}_1, \ldots, \mathcal{X}_n$, are $\alpha$-strongly convex with respect to the norms $\norm{\cdot}_1, \ldots, \norm{\cdot}_n$, respectively. Then, the function $R(x_1, \ldots, x_n) = \sum_{i=1}^n R_i(x_i)$, defined on the Cartesian product of domains, is $(\alpha/n)$-strongly convex w.r.t. the norm $\norm{(x_1, \ldots, x_n)} = \sum_{i=1}^n \norm{x_i}_i$.
\end{lemma}
\begin{proof}
Summing the definitions of strong convexity, we get
\begin{align*}
& \quad R(x_1 + h_1, \ldots, x_n + h_n) \\
&\geq \sum_{i=1}^n \langle{ \nabla R(x_i), h_i \rangle} + \fc{\al}{2}\sum_{i=1}^n \norm{h_i}_i^2 \\
&= \langle \nabla R(x_1, \ldots, x_n), \mathrm{vec}(h_{1:n}) \rangle
+ \frac{\alpha}{2} \sum_{i=1}^n \norm{h_i}_i^2 \\
&\geq \langle \nabla R(x_1, \ldots, x_n), \mathrm{vec}(h_{1:n}) \rangle+\frac{\alpha}{2n} \pa{ \sum_{i=1}^n \norm{h_i}_i }^2,
\end{align*}
where the last inequality uses the AM-QM inequality.
\end{proof}

Indeed, each term in $R(\hat\Theta)$ is strongly convex in the respective term in the composite norm $\norm{\hat\Theta}$. For $\norm{M}_{2,q}^2$ (and, identically, $\norm{N}_{2,q}^2$), we use Corollary 13 from \cite{kakade2012regularization}:
\begin{lemma}
The function $M \mapsto \norm{M}^2_{2,q}$ is $\frac{1}{3 \ln(W)}$-strongly convex w.r.t. the norm $\norm{\cdot}_{2,1}$.
\end{lemma}
This is a more general case of the fact that $\beta \mapsto \norm{\beta}_{q'}^2$ is $\frac{1}{3\ln(\tau)}$-strongly convex w.r.t. the norm $\norm{\beta}_1$.
Finally, $\sum_{j=1}^\tau \norm{P_j}_F^2$ is the squared Euclidean norm of
$\mathrm{vec}(P_{1:\tau})$, which is clearly 1-strongly convex w.r.t. the same Euclidean norm. Thus, applying Lemma~\ref{lem:multi-strongly-convex-norm}, we have:
\begin{corollary}
$R(\hat \Theta)$ is $\alpha$-strongly convex in $\norm{\hat\Theta}$, where
$\alpha = \frac{1}{12 \ln(\max(\tau,P))}.$
\end{corollary}

Finally, we note an elementary upper bound for the dual of the norm $\norm{\hat \Theta}$ in terms of the duals of the summands, which follows from the definition of dual norm:
\begin{lemma}
For any norm $\norm{\cdot}$, let $\norm{\cdot}^*$ denote its dual norm $\norm{v}^* = \sup_{\norm{w} \leq 1} \langle v,w \rangle$. Then, if $\norm{(x_1, \ldots, x_n)} = \sum_{i=1}^n \norm{x_i}_i$, we have
\[ \norm{(x_1, \ldots, x_n)}^* \leq \sum_{i=1}^n \norm{x_i}_i^*. \]
\end{lemma}
\begin{corollary}
In particular, for the norm $\norm{\hat \Theta}$ we have defined on pseudo-LDSs, we have:
\begin{align}
&\quad \norm{ (M,N,\beta,P) }^*\\
& \leq \norm{M}_{2,\infty} + \norm{N}_{2,\infty} + \norm{\beta}_\infty + \sqrt{ \sum_{j=1}^\tau \norm{P_j}_F }.
\end{align}
\end{corollary}

\subsection{Regret of the FTRL algorithm}

We state the standard regret bound of FTRL with a regularizer $R$ which is strongly convex with respect to an arbitrary norm $\norm{\cdot}$. For a reference and proof, see Theorem 2.15 in \cite{shalev2012online}.
\begin{lemma}
In the standard online convex optimization setting with decision set $\mathcal{K}$, with convex loss functions $f_1, \ldots, f_T$, let $x_{1:t}$ denote the decisions made by the FTRL algorithm, which plays an arbitrary $x_1$, then $x_{t+1} := \argmin_x \sum_{u=1}^t f_t(x) + \frac{R(x)}{\eta}$. Then, if $R(x)$ is $\alpha$-strongly convex w.r.t. the norm $\norm{\cdot}$, we have the regret bound
\[ \mathsf{Regret} := \sum_{t=1}^T f_t(x_t) - \min_x \sum_{t=1}^T f_t(x) \leq \frac{2 R_\mathrm{max}}{\eta} + \frac{\eta T}{\alpha} G_\mathrm{max}^2, \]
where $R_\mathrm{max} = \sup_{x \in \mathcal{K}} R(x)$
and $G_\mathrm{max} = \sup_{x \in \mathcal{K}} \norm{\nabla f(x)}^*$.
\end{lemma}
To optimize the bound, choose $\eta = \fc{\sqrt{2 R_\mathrm{max} T / \alpha}}{G_\mathrm{max}} $, for a regret bound of
\[ \mathsf{Regret} \leq O\pa{ G_\mathrm{max} \sqrt{R_\mathrm{max} T / \alpha} }. \]

With the facts established in Section~\ref{subsection:multi-strongly-convex}, this gives us the following regret bound, which gives an additive guarantee versus the best pseudo-LDS in hindsight:
\begin{corollary}
\label{cor:alg-rftl-regret-bound}
For the sequence of squared-loss functions on the predictions $f_1, \ldots, f_T : \mathcal{K} \rightarrow \reals$, Algorithm 1
produces a sequence of pseudo-LDSs $\hat \Theta_1, \ldots, \hat \Theta_T$ such that
\[ \sum_{t=1}^T f_t( \hat\Theta_t ) - \min_{\hat\Theta \in \mathcal{K}} \sum_{t=1}^T f_t( \hat\Theta ) \leq O \left( G R_{\hat\Theta} \sqrt{T \log \max(P,\tau)} \right), \]
where $G$ is an upper bound on the quantity
\begin{align}& \norm{\nabla_M f_t(\hat\Theta)}_{2,\infty} + \norm{\nabla_N f_t(\hat\Theta)}_{2,\infty}  \\
&+\norm{\nabla_\beta f_t(\hat\Theta)}_\infty
+ \sum_{j=1}^\tau \norm{\nabla_P f_t(\hat\Theta)}_F.\end{align}
(Here, $\nabla_M$ denotes the 4-tensor of partial derivatives with respect to the entries of $M$, and so on.)
\end{corollary}
It suffices to establish an upper bound $R_{\hat\Theta}$ on the norm of a pseudo-LDS required to approximate a true LDS, as well as the gradient of the loss function in each of these dual norms. We can obtain the appropriate diameter constraint from Theorem~\ref{thm:arma-wf}:
\[R_{\hat\Theta} = \Theta\pa{R_\Theta^2 R_\Psi R_1 \tau \sqrt{k}}.\]
We bound $G$ in the following section.

\subsection{Bounding the gradient}
In this section, we compute each gradient, and bound its appropriate norm.

\begin{lemma}
\label{lem:grad-bound}
Let $G$ be the bound in the statement in \ref{cor:alg-rftl-regret-bound}. Then,
\[ G \leq O\left( R_1^2 R_x^2 R_\Theta^2 R_\Psi R_y^2 \tau^{3/2} nk^{3/2} \log^2 T \right). \]
\end{lemma}

\begin{proof}
First, we use the result from Lemma~E.5 from \cite{HKZ17}, which states that the $\ell_1$ norm of $\phi_h$ is bounded by $O(\log T / \sigma_h^{1/4})$, to bound the size of the convolutions taken by the algorithm:
\begin{lemma}
\label{lem:filter-l1}
For any $h \in [1,k]$ and $p \in [0, W-1]$, we have
\[ \norm{ \sum_{u=1}^T \phi_h(u) \sigma_h^{1/4} \cos(2\pi u p / W) x_{t-u} }_2 \leq O\pa{ R_x \sqrt{n} \log T }. \]
The same holds upon replacing $\cos(\cdot)$ with $\sin(\cdot)$.
\end{lemma}
\begin{proof}
We have that for each coordinate $i \in [n]$,
\begin{align}
| \sum_{u=1}^T \phi_h(u) \sigma_h^{1/4} \cos(2\pi u p / W) x_{t-u}(i) | \\
\leq \sum_{u=1}^T \phi_h(u) \sigma_h^{1/4} R_x
\leq \norm{\phi_h}_1 \sigma_h^{1/4} R_x \\
\leq O\pa{ R_x \log T }.
\end{align}
\end{proof}

It will be useful to record an upper bound for the norm of the prediction residual $y(\hat\Theta) -  y_t$, which appears in the gradient of the least-squares loss.
By assumption, we have $\norm{y_t}_2 \leq R_y$.
By the constraint on $\norm{\Theta}$ from the algorithm, and noting that $y(\hat \Theta)$ a sum of matrix products of $M(p,h,:,:)$ and convolutions of the form of the LHS in Lemma~\ref{lem:filter-l1}, we can obtain a bound on $y(\hat\Theta)$ as well:
\begin{align}
\norm{ y(\hat\Theta) - y_t }_2 &\leq O\pa{ R_y \norm{ y(\hat\Theta) }_2 } \\
&\leq O\pa{R_y R_{\hat\Theta} \cdot (\sqrt{nk} \log T R_x + R_x + R_y) } \\
&\leq O \pa{ R_1^2 R_x R_\Theta^2 R_\Psi R_y^2 \tau \sqrt{n}k \log T }.
\end{align}

Call this upper bound $U$ for short.
First, we compute the gradients with respect to the 4-tensors $M$ and $N$. Fixing one phase $p$ and filter index $k$, we have:
\begin{align}
&\nabla_M f_t(\hat \Theta) (p,h,:,:) \\
=& 2 \pa{ y(\hat\Theta) - y_t }\pa{ \sum_{u=1}^T \phi_h(u) \cos(2\pi u p / W) x_{t-u} }^\top,
\end{align}
so that
\begin{align}
&\quad \norm{ \nabla_M f_t(\hat \Theta) (p,h,:,:) }_F^2 \\
&\leq 4 \norm{y(\hat\Theta) - y_t}^2 \norm{ \sum_{u=1}^T \phi_h(u) \cos(2\pi u p / W) x_{t-u} }^2 \\
&\leq U \cdot O\pa{ R_x \sqrt{n} \log T }
\end{align}
Thus, we have
\begin{align}
\norm{ \nabla_M f_t(\hat \Theta) }_{2,\infty} &= \max_{p} \sqrt{ \sum_{h=1}^k \norm{ \nabla_M f_t(\hat \Theta) (p,h,:,:) }_F^2 } \\
&\leq U \cdot O\pa{ R_x \sqrt{nk} \log T }
\end{align}
The same bound holds for $\norm{ \nabla_N f_t(\hat \Theta) }_{2,\infty}$.

For the $\beta$ part of the gradient, we have
\begin{align}
\nabla_\beta f_t(\hat \Theta) (j) = 2 \pa{ y(\hat\Theta) - y_t }^\top y_{t-j},
\end{align}
so that we have an entrywise bound of
\begin{align}
\norm{ \nabla_\beta f_t(\hat \Theta) }_\infty \leq O\pa{ R_y \cdot U }.
\end{align}

Finally, for the $P_j$ part, we have
\begin{align}
\nabla_{P_j} f_t(\hat \Theta) = 2 \pa{ y(\hat\Theta) - y_t } x_{t-j}^\top,
\end{align}
so that
\begin{align}
\sqrt{ \sum_{j=1}^\tau \norm{ \nabla_{P_j} f_t(\hat \Theta) }_F^2 } \leq O \pa{ \sqrt{\tau} R_x \cdot U }.
\end{align}

The claimed bound on $G$ follows by adding these bounds.
\end{proof}

The final regret bound follows by combining Lemma~\ref{lem:grad-bound} and Corollary~\ref{cor:alg-rftl-regret-bound}, with the choices $k = \Theta\pa{ \log T \log \pf{\tau R_\Te R_\Psi R_1R_x T}{\ep} }$, $\tau = \Theta(d), W = \Theta\pa{ \tau R_\Te^2 R_\Psi R_1R_x T^3 }$.


==> ICML18/A03-comp.tex <==
\section{Proof of main theorem: Competitive ratio bounds}
\label{app:main}
\subsection{Perturbation analysis}
To prove the main theorem, we first need to analyze the approximation when there is noise. Compared to the noiseless case, as analyzed in Theorem~\ref{thm:arma-wf-precise}, we incur an additional term equal to the size of the perturbation times a {\it competitive ratio} depending on the dynamical system.

\begin{lemma}\label{lem:perturb}
Consider an LDS $\Te=(A,B,C,h_0=0)$ that satisfies the conditions of Theorem~\ref{thm:arma-wf}. 
%and let $(M,N, \be,P)$ be chosen as in the theorem.
Consider the LDS under adversarial noise~\eqref{eq:lds-noise1}--\eqref{eq:lds-noise2}. Let $y_{t}(x_{1:T}, \eta_{1:T},\xi_{1:T})$ be the output at time $t$ given inputs $x_{1:T}$ and noise $\eta_{1:T},\xi_{1:T}$.  Let $\hat y_t(x_{1:T},\eta_{1:T},\xi_{1:T})$ be the prediction made by the pseudo-LDS at time $t$. 
%Given inputs $x_1,\ldots, x_T$, let the outputs be $y_1^*,\ldots, y_T^*$. 
Suppose that $(M,N,-\be,P)$ is a pseudo-LDS that predicts well when there is no noise: %if $\hat y_t$ is the prediction at time $t$,
\begin{align}
&\quad \ve{\hat y_{1:T}(x_{1:T},0,0) - y_{1:T}(x_{1:T},0,0)}_2\\
&=\pa{\sumo tT \ve{\hat y_t(x_{1:T},0,0)  - y_t^*(x_{1:T},0,0) }_2^2}^{\rc 2}\le \ep.
\end{align}
%Now consider the same LDS but under adversarial noise~\eqref{eq:lds-noise1}--\eqref{eq:lds-noise2} satisfying $\sumo tT \ve{\eta_t}^2 + \ve{\xi_t}^2\le L$. Given inputs $x_1,\ldots, x_T$, let $y_1,\ldots, y_T$ be the outputs of this system. 
For bounded adversarial noise $\sumo tT \ve{\eta_t}^2 + \ve{\xi_t}^2\le L$,
\begin{align}
& \quad \ve{\hat y_{1:T}(x_{1:T},\eta_{1:T},\xi_{1:T}) - y_{1:T}(x_{1:T},\eta_{1:T},\xi_{1:T})}_2 \\
&\le \ep + O(\ve{\be}_\iy \tau^{\fc 32} R_\Te R_\Psi \sqrt L).
%\sumo tT \ve{y(M,N,\be,P_{0:\tau-1}, x_{1:t},y_{t-1:t-\tau}) - y_t}^2\le (\ep+\ve{\be}_\iy \tau^{\fc 32} R_\Te L)^2.
\end{align}
\end{lemma}
Note that the initial hidden state can be dealt with by considering it as noise in the first step $\eta_1$.
\begin{proof}
Note that $\hat y_t$ is a linear function of $x_{1:T},\eta_{1:T}, \xi_{1:T}$.
\begin{align}
& \quad \hat y_t(x_{1:T},\eta_{1:T},\xi_{1:T})-y_t \\
&= [\hat y_t(0,0,\xi_{1:T}) - y_t(0,0,\xi_{1:T})]\\
 &\quad + [\hat y_t(0,\eta_{1:T},0) - y_t(0,\eta_{1:T},0)] \\
 &\quad + [\hat y_t(x_{1:T}, 0,0) - y_t(x_{1:T}, 0,0) ].\label{eq:perturb0}
\end{align}
%Consider the error $\sqrt{\sumo tT\ve{\hat y_t - y_t^*}^2}$. Because the predictions $\hat y_t$ respond linearly to $\eta_t, \xi_t$, this error is at most the sum of the errors incurred by each $\eta_t$ and $\xi_t$ individually.
This says that the residual is the sum of the residuals incurred by each $\xi_t$ and $\eta_t$ individually, plus the residual for the non-noisy LDS, $\hat y_t(x_{1:T}, 0,0) - y_t(x_{1:T}, 0,0)$.

We first analyze the effect of a single perturbation to the observation $\xi_t$. Suppose $\eta_t=0$ for all $t$ and $\xi_t=0$ except for $t=u$ (so that $y_t=0$ for all $t$ except $t=u$, where $y_u=\xi_u$). The predictions $\hat y_t$ are zero when $t\nin [u, u+\tau]$, because then the prediction does not depend on $y_u$. For $u\le t\le u+\tau$,
%\hl{be consistent with sign of $\be$}
\begin{align}
&\quad \ve{\hat y_t(0,0,\xi_{1:T}) - y_t(0,0,\xi_{1:T})}_2 \\
&=
\ve{y_t + \sumo j{\tau}\be_j y_{t-j}}_2\\
%&= \max_{0\le j\le \tau}\ve{\be_j}_2\\
&\le |\be_{t-u}| \ve{\xi_{u}}_2\\
&\quad \ve{\hat y_{1:T}(0,0,\xi_{1:T})-y_{1:T}(0,0,\xi_{1:T})}_2\\
&\le\pa{\sum_{t=u}^{u+\tau} |\be_{t-u}|^2}^{\rc 2} \ve{\xi_u}_2\\
%\sqrt{\sumo tT\ve{y_t - \hat y_t}_2^2}&
&=\ve{\be}_2\ve{\xi_u}_2.\label{eq:perturb1}
\end{align}

Now we analyze the effect of a single perturbation to the hidden state $\eta_t$. Suppose $\xi_t=0$ for all $t$ and $\eta_t=0$ except for $t=u$ (so that $h_t=0$ for all $t<u$, $h_u=\eta_u$, and the system thereafter evolves according to the LDS). 
For simplicity, we may as well consider the case where $u=1$, i.e., the perturbation is to the initial hidden state.
When $t\le \tau$, the error is bounded by 
%When $u\le t< u+\tau$, the error is bounded by
\begin{align}
&\quad \ve{\hat y_t(0,\eta_{1:T},0)- y_t(0,\eta_{1:T},0)}_2\\
&=\ve{y_t + \sumo j{t-1}\be_j y_{t-j}}_2
= \ve{C \sumz j{t-1}\be_j A^{t-j-1}\xi_1}\\
&\le \ve{C}_2 \ve{\be}_1 \ve{\Psi}_F \ve{\La}_2 \ve{\Psi^{-1}}_F\ve{\eta_1}_2\\
&\le R_\Te R_\Psi \ve{\be}_1 \ve{\eta_1}_2\\
&\quad \ve{\hat y_{1:\tau}(0,\eta_{1:T},0)-\hat y_{1:\tau}(0,\eta_{1:T},0)}_2 \\
&\le \tau^{\rc 2} R_\Te R_\Psi \ve{\be}_1 \ve{\eta_1}_2.\label{eq:perturb2}
\end{align}

When $t>\tau$, %u+\tau
the error is (let $\be_0=1$)
\begin{align}
%\ve{y_t - \hat y_t}_2
&\quad y_t(0,\eta_{1:T},0)-
\hat y_t(0,\eta_{1:T},0)\\
&= {C \sumz j{\tau}\be_j A^{t-j-1}\eta_1}\\
&\le C\sumz{j}{\tau} \sumo{\ell}d \be_j \al_\ell^{t-j-1} v_\ell w_\ell^* \eta_1\\
&= C\sumz{j}{\tau} \sumo{\ell}d \be_j \al_\ell^{t-\tau-1} (\al_\ell^{\tau-j} - \om_\ell^{\tau-j}) v_\ell w_\ell^* \eta_1\\
&= C\sumo{j}{\tau} \sumo{\ell}d \be_j \om_\ell^{t-j}r_\ell^{t-\tau-1} (r_\ell^{\tau-j}-1) v_\ell w_\ell^* \eta_1\\
%%
&\quad \ve{\hat y_t(0,\eta_t,0)-y_t(0,\eta_{1:T},0)}_2 \\
&\le \ve{\be}_\iy \sumo j{\tau}\sumo{\ell}d 
\fc{1-r_\ell^{\tau-j}}{1-r_\ell}\mu(r_\ell)_{t-\tau} \ve{C v_\ell w_\ell^* \eta_1}_2\\
&\le  \ve{\be}_\iy  R_\Te \ve{\eta_1}_2\sumo j{\tau}\sumo{\ell}d 
\fc{1-r^{\tau-j}}{1-r}\mu(r_\ell)_{t-\tau}\ve{v_\ell w_\ell^* }_2\\
%%
&\quad\ve{\hat y_{\tau+1:T}(0,\eta_{1:T},0)-y_{\tau+1:T}(0,\eta_{1:T},0)}_2\\
&\le \ve{\be}_\iy R_\Te \ve{\eta_1}_2 \sumo j{\tau} \max_{r,\ell} \ve{\fc{1-r_\ell^{\tau-j}}{1-r_\ell}\mu(r_\ell)}_2 R_\Psi\\
&\le \ve{\be}_\iy R_\Te \ve{\eta_1}_2 \pa{\sumo j{\tau} \sqrt{\tau-j}}R_\Psi\\
&\le \ve{\be}_\iy R_\Te R_\Psi \tau^{\fc 32}\ve{\eta_1}_2\label{eq:perturb3}
\end{align}
by the calculation in~\eqref{eq:RPsi} and~\eqref{eq:L-bound} because 
\begin{align}
&\quad \ve{\fc{1-r^{k}}{1-r}\mu(r)}_2\\
&\le (1-r^k)\sfc{1}{1-r^2}\le 
\min\{1,k(1-r)\} \sfc{1}{1-r}\\
&=\min\bc{\sfc{1}{1-r}, k\sqrt{1-r}}\le \sqrt k.
\end{align}
%The total error $\hat y_t-y_t$ 
%is the sum of the errors accrued by the $\eta_t$ and $\xi_t$, plus the error in approximating the noiseless system, $\hat y_t-y_t^*$.
Combining~\eqref{eq:perturb1},~\eqref{eq:perturb2}, and~\eqref{eq:perturb3} using~\eqref{eq:perturb0} and noting $\ve{\be}_1\le(\tau+1)\ve{\be}_\iy$ gives
\begin{align}
&\quad \ve{\hat y_{1:T}(x_{1:T}, \eta_{1:T},\xi_{1:T})-y_t}_2\\
 &\le 
\ve{\be}_2 \ve{\eta}_2
+R_\Te R_\Psi \sqrt{\tau}
( \ve{\be}_1 + \ve{\be}_\iy  \tau) \ve{\xi}_2 + \ep\\
&\le O(\ve{\be}_\iy\tau^{\fc 32} R_\Te R_\Psi \sqrt{L})+\ep
%\ve{\be}_\iy R_\Te\tau^{\fc 32}\ve{\eta}_2
%+\ep \le \ve{\be}_\iy R_\Te \tau^{\fc 32} L+\ep.
\end{align}
\end{proof}


\subsection{Proof of Main Theorem}
\label{app:main-pf}
We prove Theorem~\ref{thm:main} with the following more precise bounds. 


\begin{theorem}\label{thm:main-formal}
Consider a LDS with noise satisfying the assumptions in Section~\ref{sec:setting} (given by~\eqref{eq:lds-noise1} and~\eqref{eq:lds-noise2}), where total noise is bounded by $L$. 
Then there is a choice of parameters such that
%with parameters $k=O\pa{\poly\log\pa{T, R_\Te, R_\Psi, R_1, R_x, \rc{\ep}}}$, $P=O\pa{\poly(\tau, R_\Te, R_\Psi, R_1, R_x, T)}$, 
%\hl{what is the regularization weight?} 
Algorithm~\ref{alg:asym-lds} learns a pseudo-LDS $\hat \Te$ whose predictions $\hat y_t$ satisfy
\begin{align}\label{eq:main-formal}
\sumo{t}T \ve{\hat y_t - y_t}^2 &\le 
\tilde{O}\pa{R d^{5/2} n \sqrt{T}} + 
O(R_\iy^2 \tau^{3} R_\Te^2 R_\Psi^2 L)
\end{align}
where the $\tilde O(\cdot)$ only suppresses factors polylogarithmic in $n,m,d,R_\Theta,R_x,R_y,\log T$, and $R_1^3 R_x^2 R_\Theta^4 R_\Psi^2 R_y^2\leq R$.
\end{theorem}
\begin{proof}
Consider the fixed pseudo-LDS which has smallest total squared-norm error in hindsight for the noiseless LDS. Let $y_t^*(x_{1:T},\eta_{1:T},\xi_{1:T})$ denote its predictions under inputs $x_{1:T}$ and noise $\eta_{1:T},\xi_{1:T}$ and $y_t(x_{1:T},\eta_{1:T},\xi_{1:T})$ denote the true outputs of the system.
Given $\ep>0$, choosing $k,P$ as in  Theorem~\ref{thm:arma-wf-precise} (Approximation) gives
\begin{align}
\forall 1<t<T,\quad \ve{y_t^*(x_{1:T},0,0)-
y_t(x_{1:T},0,0)}_2
&\le \ep\\
\implies  \ve{y_{1:T}^*(x_{1:T},0,0)-
y_{1:T}(x_{1:T},0,0)}_2
&\le \ep\sqrt T.
\end{align}
By Lemma~\ref{lem:perturb} (Perturbation),
\begin{align}
&\quad \ve{y_{1:T}^*(x_{1:T},\eta_{1:T},\xi_{1:T})-
y_t(x_{1:T},\eta_{1:T},\xi_{1:T})}_2\\
&\le \ep \sqrt T + O(R_\iy \tau^{\fc 32} R_\Te R_\Psi \sqrt L)\label{eq:main-perturb}
\end{align}

%Let $y_1^*,\ldots, y_T^*$ denote the predictions made by the fixed pseudo-LDS which has the smallest total squared-norm error in hindsight. We use the notation $\ve{a_{1:T}}^2:= \sumo tT a_t^2$ as in Lemma~\ref{lem:perturb}. 
In the below we consider the noisy LDS (under inputs $x_{1:T}$ and noise $\eta_{1:T},\xi_{1:T}$). 
By Theorem~\ref{thm:regret} (Regret) and~\eqref{eq:main-perturb},
\begin{align}
&\quad \ve{\hat y_{1:T} - y_{1:T}}_2^2\\
&= (
\ve{\hat y_{1:T} - y_{1:T}}_2^2 - 
\ve{\hat y_{1:T}^* - \hat y_{1:T}}_2^2 
)
+\ve{\hat y_{1:T}^* - y_{1:T}}_2^2\\
&\le 
\tilde
O\pa{R_1^3 R_x^2 R_\Theta^4 R_\Psi^2 R_y^2 d^{5/2} n \log^7 T \sqrt{T}} \\ & + 
 \ep^2 T + O(R_\iy^2 \tau^{3} R_\Te^2 R_\Psi^2 L)
\end{align}
Choosing $\ep={T^{-\rc 4}}$ (and $k,P$ based on $\ep$) means $\ep^2T$ is absorbed into the first term, and we obtain the bound in the theorem.
\end{proof}



==> ICML18/defs.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{example}[theorem]{Example}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{application}[theorem]{Application}
\newtheorem{optimizationproblem}[theorem]{Optimization~Problem}

\newcommand{\todo}[1]{\textbf{\textcolor{red}{TODO: #1}}}

\def\mO{{\mathcal O}}
\def\D{{\mathcal D}}
\def\L{{\mathcal L}}
\def\F{{\mathcal F}}
\def\mP{{\mathcal P}}
\def\reals{{\mathbb R}}
\def\R{{\mathcal R}}
\def\fhat{{\ensuremath{\hat{f}}}}

\DeclareMathOperator{\clip}{clip}
\def\norm#1{\mathopen\| #1 \mathclose\|}% use instead of $\|x\|$

\newcommand{\ellipsoid}{{\mathcal E}}
\newcommand{\sround}{\mathop{\mbox{\rm SmartRound}}}
\newcommand{\round}{\mathop{\mbox{\rm round}}}
\newcommand{\myspan}{\mathop{\mbox{\rm span}}}
\newcommand{\edges}{\mathop{\mbox{\rm edges}}}
\newcommand{\conv}{\mathop{\mbox{\rm conv}}}
\newcommand{\sign}{\mathop{\mbox{\rm sign}}}
\newcommand{\poly}{\mathop{\mbox{\rm poly}}}
\newcommand{\rank}{\mathop{\mbox{\rm rank}}}

\newcommand{\ignore}[1]{}
\newcommand{\equaldef}{\stackrel{\text{\tiny def}}{=}}
\newcommand{\equaltri}{\triangleq}
\newcommand{\tr}{\ensuremath{{\scriptscriptstyle\mathsf{T}}}}
\def\trace{{\bf Tr}}
\def\dist{{\bf P}}
\def\mydist{{\bf Q}}
\def\reals{{\mathbb R}}
\newcommand\E{\mbox{\bf E}}
\newcommand\ball{\mathbb{B}}
\newcommand\var{\mbox{VAR}}
\def\bzero{\mathbf{0}}

\def\Exp{\mathop{\mbox{E}}}
\def\mP{{\mathcal P}}
\def\risk{{\mbox{Risk}}}
\def\ent{{\mbox{ent}}}
\def\mG{{\mathcal G}}
\def\mA{{\mathcal A}}
\def\V{{\mathcal V}}
\def\lhat{\hat{\ell}}
\def\Lhat{\hat{L}}
\def\ltil{\tilde{\ell}}
\def\Ltil{\tilde{L}}

\def\Ahat{\hat{\mathbf{A}}}

\def\bold0{\mathbf{0}}
\def\boldone{\mathbf{1}}
\def\boldp{\mathbf{p}}
\def\boldq{\mathbf{q}}
\def\boldr{\mathbf{r}}
\def\boldA{\mathbf{A}}
\def\boldI{\mathbf{I}}
\newcommand\mycases[4] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4}
\end{array}
\right. }}
\newcommand\mythreecases[6] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4} \\\\
    {#5} & {#6}
\end{array}
\right. }}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\be{\mathbf{e}}
\def\etil{\tilde{\mathbf{e}}}
\def\bk{\mathbf{k}}
\def\bu{\mathbf{u}}
\def\bx{\mathbf{x}}
\def\w{\mathbf{w}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}

\def\bw{\mathbf{w}}
\def\ba{\mathbf{a}}
\def\bA{\mathbf{A}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bV{\mathbf{V}}
\def\bone{\mathbf{1}}


\def\xhat{\hat{\mathbf{x}}}
\def\xbar{\bar{\mathbf{x}}}
\def\vol{\mbox{vol}}
\def\trace{{\bf Tr}}
\def\Exp{\mathop{\mbox{E}}}
\newcommand{\val}{\mathop{\mbox{\rm val}}}
\renewcommand{\deg}{\mathop{\mbox{\rm deg}}}
\newcommand{\eps}{\varepsilon}

% Macros for this chapter
\def\bone{\mathbf{1}}
\newcommand{\sphere}{\ensuremath{\mathbb {S}}}
\newcommand{\simplex}{\ensuremath{\Delta}}
\newcommand{\diag}{\mbox{diag}}
\newcommand{\K}{\ensuremath{\mathcal K}}
\newcommand{\Ktil}{\ensuremath{\mathcal{\tilde{K}}}}
\def\mA{{\mathcal A}}
\newcommand{\x}{\ensuremath{\mathbf x}}
\newcommand{\rv}[1][t]{\ensuremath{\mathbf r_{#1}}}
\newcommand{\y}{\ensuremath{\mathbf y}}
\newcommand{\z}{\ensuremath{\mathbf z}}
\newcommand{\h}{\ensuremath{\mathbf h}}
\newcommand{\xtil}[1][t]{\ensuremath{\mathbf {\tilde{x}}_{#1}}}
\newcommand{\xv}[1][t]{\ensuremath{\mathbf x_{#1}}}
\newcommand{\xvh}[1][t]{\ensuremath{\mathbf {\hat x}}_{#1}}
\newcommand{\ftildeh}[1][t]{\ensuremath{\mathbf {\hat f}}_{#1}}
\newcommand{\xvbar}[1][t]{\ensuremath{\bar{\mathbf x}_{#1}}}
\newcommand{\xstar}{\ensuremath{\mathbf x^{*}}}
\newcommand{\xstarr}{\ensuremath{\mathbf x^{\star}}}
\newcommand{\yv}[1][t]{\ensuremath{\mathbf y_{#1}}}
\newcommand{\zv}[1][t]{\ensuremath{\mathbf z_{#1}}}
\newcommand{\fv}[1][t]{\ensuremath{\mathbf f_{#1}}}
\newcommand{\gv}[1][t]{\ensuremath{\mathbf g_{#1}}}
\newcommand{\qv}[1][t]{\ensuremath{\mathbf q_{#1}}}
\newcommand{\pv}[1][t]{\ensuremath{\mathbf p_{#1}}}
\newcommand{\ftilde}[1][t]{\ensuremath{\mathbf {\tilde f}_{#1}}}
\newcommand{\gtilde}[1][t]{\ensuremath{\mathbf {\tilde g}_{#1}}}
\newcommand{\lowtrace}{\mathcal{T}}

\newcommand{\ev}[1][i]{\ensuremath{\mathbf e_{#1}}}
\newcommand{\uv}{\ensuremath{\mathbf u}}
\newcommand{\ww}{\ensuremath{\mathbf w}}
\newcommand{\vv}{\ensuremath{\mathbf v}}
\newcommand{\A}[1][t]{\ensuremath{\mathbf A_{#1}}}
\newcommand{\Ftilde}[1][t]{\ensuremath{\mathbf {\tilde F}_{#1}}}
\newcommand{\Gtilde}[1][t]{\ensuremath{\mathbf {\tilde G}_{#1}}}
\newcommand{\hessum}[1][t]{\ensuremath{\boldsymbol{H}_{1:#1}}}
\newcommand{\reg}[1][t]{\ensuremath{\lambda_{#1}}}
\newcommand{\regsum}[1][t]{\ensuremath{\boldsymbol{\lambda}_{1:#1}}}
\newcommand{\bM}{\ensuremath{\mathcal M}}
%\newcommand{\F}{\ensuremath{\mathcal F}}
\newcommand{\ntil}{\tilde{\nabla}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\rhotil}{\tilde{\rho}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\mutil}{\tilde{\mu}}
\newcommand{\Atil}{\tilde{A}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\vtil}{\tilde{v}}
\newcommand\super[1] {{^{(#1)}}}
\newcommand\pr{\mbox{\bf Pr}}
\newcommand\av{\mbox{\bf E}}
\def\regret{\ensuremath{\mbox{Regret}}}
\def\bb{\mathbf{b}}
%\def\bB{\mathbf{B}}
\def\bB{{B}}
%\def\bC{\mathbf{C}}
\def\bC{{C}}
\def\bS{{S}}
\def\be{\mathbf{e}}
\def\bu{\mathbf{u}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bdelta{\mathbf{\delta}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bv{\mathbf{v}}
\def\ba{\mathbf{a}}
%\def\bA{\mathbf{A}}
\def\bA{{A}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bV{\mathbf{V}}
\def\sgn{\text{sgn}}
\def\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\tsum{{\textstyle \sum}}
\def\universal{{\sc Universal}\xspace}
\def\ogd{{\sc Online Gradient Descent}\xspace}
\def\R{\ensuremath{\mathcal R}}


